Safe Navigation and Obstacle Avoidance Using Differentiable Optimization Based Control Barrier Functions

Control barrier functions (CBFs) have been widely applied to safety-critical robotic applications. However, the construction of control barrier functions for robotic systems remains a challenging task. Recently, collision detection using differentiable optimization has provided a way to compute the minimum uniform scaling factor that results in an intersection between two convex shapes and to also compute the Jacobian of the scaling factor. In this letter, we propose a framework that uses this scaling factor, with an offset, to systematically define a CBF for obstacle avoidance tasks. We provide theoretical analyses of the continuity and continuous differentiability of the proposed CBF. We empirically evaluate the proposed CBF's behavior and show that the resulting optimal control problem is computationally efficient, which makes it applicable for real-time robotic control. We validate our approach, first using a 2D mobile robot example, then on the Franka-Emika Research 3 (FR3) robot manipulator both in simulation and experiment.

==> cont_diff_proof.tex <==
Next, under sufficient conditions, we show that $\alpha^\star$ is continuously differentiable with respect to $\psi$.
\begin{defn}[Scaling Function]
\label{def:scaling_func}
    We say that $\mathcal{F}_A: \mathbb{R}^3 \rightarrow \mathbb{R}$,  is a scaling function for an object $A \subset \mathbb{R}^3$, if it is a continuously differentiable convex function, then $\mathcal{F}_A(p) \geq 0$, $A = \{p \mid \mathcal{F}_A(p) \leq 1\}$, $\partial A = \{p \mid \mathcal{F}_A(p) = 1\}$, and $\min_p\mathcal{F}_A(p) = 0$.
\end{defn}
\noindent For example, the scaling function for an ellipsoid $A$ has form $\mathcal{F}_A = (p - r)^\top\mathbf{P}(p - r)$ where $\mathbf{P} \in \mathbb{R}^3$ is a diagonal matrix with inverses of squared semi-axes lengths on its diagonal. This particular example is used in~\cite{TracyHM22} to implement the scaling constraint for the ellipsoid, and similar functions can be derived for other shapes discussed in~\cite{TracyHM22}.
\begin{lem}
\label{lem:scaling}
    For two objects $A, B \subset \mathbb{R}^3$, denote their scaling functions as $\mathcal{F}_A$ and $\mathcal{F}_B$, respectively. If $\mathcal{F}_A$ and $\mathcal{F}_B$ are differentiable functions, and no point $p$ exists such that $\partial\mathcal{F}_A/\partial p = \partial\mathcal{F}_B/\partial p = \mathbf{0}$, then for the optimal solution $(p^\star, \alpha^\star)$ of~\eqref{eq:differentiable_collision}, we have $\mathcal{F}_A(p^\star) = \mathcal{F}_B(p^\star) = \alpha^\star$ and $\nu_A^\star, \nu_B^\star \neq 0$.
\end{lem}
\begin{proof}
    First, we rewrite the problem in~\eqref{eq:differentiable_collision} as
    \begin{equation}
    \label{eq:scaling_opt}
        \min_{p, \alpha}\ \alpha\ \mathrm{subject\ to}\ \mathcal{F}_A(p) \leq \alpha, \mathcal{F}_B(p) \leq \alpha, \alpha > 0.
    \end{equation}
    Then, we have part of the KKT conditions as
    \begin{subequations}
    \begin{align}
        \label{eq:lem_kkt_1}
        \nu_A^\star + \nu_B^\star &= 1\\
        \label{eq:lem_kkt_2}
        \nu_A^\star\frac{\partial\mathcal{F}_A}{\partial p}(p^\star) + \nu_B^\star\frac{\partial\mathcal{F}_B}{\partial p} &= 0\\
        \label{eq:lem_kkt_3}
        \nu_A^\star(\mathcal{F}_A(p^\star) - \alpha^\star) &= 0\\
        \label{eq:lem_kkt_4}
        \nu_B^\star(\mathcal{F}_B(p^\star) - \alpha^\star) &= 0.
    \end{align}
    \end{subequations}
    It can be shown that neither $\nu_A^\star$ nor $\nu_B^\star$ can be 0. To show this, without loss of generality, assume $\nu_A^\star = 0$. From~\eqref{eq:lem_kkt_1}, we have $\nu_B^\star = 1$ and from~\eqref{eq:lem_kkt_2} we have $\nabla_p\mathcal{F}_B(p^\star) = 0$. From definition~\ref{def:scaling_func}, we know that $\mathcal{F}_B$ is a convex differentiable function, therefore, $p^\star$ is the global minimum of $\mathcal{F}_B$. Hence, also from definition~\ref{def:scaling_func}, $\mathcal{F}_B(p^\star) = 0$. Then, from~\eqref{eq:lem_kkt_4}, $\alpha^{\star} = \mathcal{F}_B(p^\star) = 0$. Using the constraint $\mathcal{F}_A(p) \leq \alpha$ from~\eqref{eq:scaling_opt} and the condition $\mathcal{F}_A(p) \geq 0$ from definition~\eqref{def:scaling_func}, we have $\mathcal{F}_A(p^\star) = 0$, which means $p^\star$ is also a global minimizer for $\mathcal{F}_A$, i.e., $\partial\mathcal{F}_A(p^\star)/\partial p = \mathbf{0}$. Since, by the assumption of Lemma~\ref{lem:scaling}, no point $p$ exists such that $\partial\mathcal{F}_A/\partial p = \partial\mathcal{F}_B/\partial p = \mathbf{0}$, thus, $\nu_A^\star \neq 0$. Given the symmetry between $\nu_A^\star$ and $\nu_B^\star$, $\nu_B^\star \neq 0$. Therefore, from~\eqref{eq:lem_kkt_3} and~\eqref{eq:lem_kkt_4}, we have $\mathcal{F}_A(p^\star) = \mathcal{F}_B(p^\star) = \alpha$.
\end{proof}

\begin{thm}
\label{thm:cont_diff}
    Consider two parameterized scaling functions $\mathcal{G}_A(p,\psi) = \mathcal{F}_{A(\psi)}(p)$ and $\mathcal{G}_B(p,\psi) = \mathcal{F}_{B(\psi)}(p)$ such that, for any $\psi \in \Psi$, these are scaling functions  for varying sets $A(\psi), B(\psi) \subset \mathbb{R}^3$. Furthermore, for all $p$ and $\psi$, assume that the conditions of Lemma~\ref{lem:scaling} holds, $\mathcal{G}_A$ and $\mathcal{G}_B$ are strongly convex on $p$, the gradients $\partial\mathcal{G}_A/\partial\psi$ and $\partial\mathcal{G}_B/\partial\psi$ and the Hessians $\partial^2\mathcal{G}_A/\partial p^2$, $\partial^2\mathcal{G}_A/\partial p\partial\psi$, $\partial^2\mathcal{G}_B/\partial p^2$, and $\partial^2\mathcal{G}_B/\partial p\partial\psi$ are continuous in $\psi$, then, $\alpha^\star(\psi)$ is continuously differentiable w.r.t. $\psi$.
\end{thm}
\begin{proof}
    From~\eqref{eq:lem_kkt_1}, we have
        $\partial\nu_A^\star/\partial\psi + \partial\nu_B^\star/\partial\psi = 0$.
    Then, using Lemma~\ref{lem:scaling}, and taking the partial derivative with respect to $\psi$ on both sides of~\eqref{eq:lem_kkt_1} and~\eqref{eq:lem_kkt_2}, we obtain
    \begin{equation}
    \label{eq:linear_equations}
        \underbrace{\begin{bmatrix}
            \mathbf{M} & \mathbf{c}\\
            \mathbf{c}^\top & \mathbf{0}
        \end{bmatrix}}_{\mathbf{N}}\begin{bmatrix}
            \displaystyle\Big(\frac{\partial p^\star}{\partial\psi}\Big)^\top & \displaystyle\Big(\frac{\partial\nu_A^\star}{\partial\psi}\Big)^\top
        \end{bmatrix}^\top = \begin{bmatrix}
            \Omega_1\\
            \Omega_2
        \end{bmatrix}
    \end{equation}
    with
    \begin{subequations}
    \begin{align}
        \label{eq:thm_eq_1}
        \mathbf{M} &= \frac{\partial^2\mathcal{G}_A}{\partial p^2}(p^\star, \psi)\nu_A^\star + \frac{\partial^2\mathcal{G}_B}{\partial p^2}(p^\star, \psi)\nu_B^\star\\
        \label{eq:thm_eq_2}
        \mathbf{c} &= \frac{\partial\mathcal{G}_A}{\partial p}(p^\star, \psi) - \frac{\partial\mathcal{G}_B}{\partial p}(p^\star, \psi)\\
        \label{eq:thm_eq_3}
        \Omega_1 &= -\frac{\partial^2\mathcal{G}_A}{\partial p\partial\psi}(p^\star, \psi)\nu_A^\star - \frac{\partial^2\mathcal{G}_B}{\partial p\partial\psi}(p^\star, \psi)\nu_B^\star\\
        \label{eq:thm_eq_4}
        \Omega_2 &= \frac{\partial\mathcal{G}_B}{\partial\psi}(p^\star, \psi) - \frac{\partial\mathcal{G}_A}{\partial\psi}(p^\star, \psi).
    \end{align}
    \end{subequations}
    Since $\mathcal{G}_A$ and $\mathcal{G}_B$ are strongly convex and $\nu_A^\star$ and $\nu_B^\star$ are dual feasible and thus strictly positive from Lemma~\ref{lem:scaling}, $\mathbf{M} \succ 0$. Note that $\mathbf{c} = \mathbf{0}$ would imply from \eqref{eq:lem_kkt_1} and \eqref{eq:lem_kkt_2} that $\partial\mathcal{G}_A(p^\star, \psi)/ \partial p = \partial\mathcal{G}_B(p^\star, \psi)/ \partial p = 0$, violating the condition of Lemma~\ref{lem:scaling}. Hence, $\mathbf{c} \neq \mathbf{0}$. Then, using Schur complement, we can conclude that the matrix $\mathbf{N}$ is invertible. Since, $\mathbf{M}$, $\mathbf{c}$, $\Omega_1$, and $\Omega_2$ are continuous in $\psi$, $\mathbf{N}^{-1}$ is continuous on $\psi$, thus, $\partial p^\star/\partial\psi$ is also continuous in $\psi$. Then, from Lemma~\ref{lem:scaling},
    \begin{equation}
        \frac{\partial\alpha^\star}{\partial\psi}(\psi) = \frac{\partial\mathcal{G}_A}{\partial p}(p^\star, \psi)\frac{\partial p^\star}{\partial\psi}(\psi) + \frac{\partial\mathcal{G}_A}{\partial\psi}(p^\star, \psi)
    \end{equation}
    which, following the above derivation, is continuous.
\end{proof}
\begin{rem}
    For ellipsoids/spheres, we can write a scaling function (as noted after Definition~\ref{def:scaling_func}) that satisfies Theorem~\ref{thm:cont_diff}.
\end{rem}

Based on empirical studies, we believe that continuous differentiability holds under more general conditions motivating Conjecture~\ref{conj:cbf_condition}.

\begin{conj}
\label{conj:cbf_condition}
Assume we have two convex objects $A$ and $B$. If $A$ is a strongly convex object (e.g., ellipsoid, sphere) and $B$ is a convex object that can either have a non-smooth surface (e.g., cylinder, polygon, cone) or a smooth surface, then the CBF defined in~\eqref{eq:diffopt_cbf} is continuously differentiable.
\end{conj}

==> new_proof.tex <==
To show~\eqref{eq:diffopt_cbf} is a valid CBF, we need to show continuous differentiability of $\alpha^\star$. In this paper, we prove continuity of $\alpha^\star$ in the general case and then prove continuous differentiability for the case of strongly convex scaling function when the gradients and Hessians exist and are continuous. We conjecture that continuous differentiability can be generalized to one object being strongly convex and the second being only convex although a formal proof is still elusive. 
% First, we state one of the main theoretical results.
% Theorem 1
\begin{thm}
\label{thm:main}
The optimal value of~\eqref{eq:differentiable_collision}, denoted as $\alpha^\star$, is a continuous function with respect to the positions and orientations of $A$ and $B$.
\end{thm}

To prove Theorem~\ref{thm:main}, we need  Lemma~\ref{lem:compact_correspondence} with the constraint correspondence $\Gamma(\psi)$ defined as
\begin{equation}
    \Gamma(\psi) = \{(p, \alpha)\mid p \in \mathcal{P}_{AB}(\alpha \mid \psi), \alpha \in S\}
    \label{eq:constraint_correspondence}
\end{equation}
with $S \subset \mathbb{R}$ being a compact set and $\mathcal{P}_{AB}(\alpha \mid \psi) = \mathcal{P}_{A}(\alpha \mid \psi) \cap \mathcal{P}_B(\alpha \mid \psi)$. Also we define $\Gamma_i(\psi) = \{(p,\alpha) \mid p\in\mathcal{P}_i(\alpha\mid\psi), \alpha \in S\}$ with $i \in \{A, B\}$. We can then show that $\Gamma(\psi)$ is a compact-valued correspondence on $\mathbb{R}^4$.

\begin{lem}
\label{lem:compact_correspondence}
The constraint correspondence $\Gamma(\psi)$ defined in~\eqref{eq:constraint_correspondence} is a compact-valued correspondence.
\end{lem}
\begin{proof}
First, we show that $\Gamma_A(\psi)$ is a compact-valued correspondence. Define $K_A(\psi) = \mathcal{P}_A(1\mid\psi) \subset \mathbb{R}^3$, and the function $\phi: K_A(\psi) \times S \rightarrow \mathbb{R}^4$ as $\phi(p, \alpha) = (\alpha(p - r_1) + r_1, \alpha)$, which is a continuous function on $K_A(\psi) \times S$. Because both $K_A(\psi)$ and $S$ are compact sets, we have $K_A(\psi) \times S$ as a compact set on $\mathbb{R}^4$. Since the image of $\psi$ under $\Gamma_A$ is the same as the image of $K_A(\psi) \times S$ under $\phi$, using the property that continuous functions map compact sets to compact sets, and $K_A(\psi)$ is a compact set for any value of $\psi$, we have $\Gamma_A(\psi)$ being a compact-valued correspondence. Using the same logic, for all $\psi$, $\Gamma_B(\psi)$ is also a compact-valued correspondence. Since $\Gamma(\psi) = \Gamma_A(\psi) \cap \Gamma_B(\psi)$, and intersections of compact sets are compact sets, we can conclude that $\Gamma(\psi)$ is a compact-valued correspondence.
\end{proof}

We can directly apply Theorem~\ref{thm:berge} to prove Theorem~\ref{thm:main} if we show that $\Gamma(\psi)$ is both UHC and LHC. 

\begin{proof}
\textbf{(Theorem~\ref{thm:main})} To show UHC, we consider an arbitrary open set $V$ such that  $\Gamma(\psi) \subset V$, i.e.,
\begin{equation}
    V = \Big\{(p, \alpha) \mid \mathcal{P}_{AB}(\alpha \mid \psi) \subset V_p(\alpha), S \subset V_\alpha\Big\}
\end{equation}
with $V_p$ being an open set on $\mathbb{R}^3$, $p \in \mathcal{P}_{AB}(\alpha \mid \psi)$, $V_\alpha$ being an open set on $\mathbb{R}$, and $\alpha \in S$. In our case, UHC is equivalent to: for any $\psi$ and $\alpha$, if the intersection of the two convex shapes $\mathcal{P}_A$ and $\mathcal{P}_B$ is contained within an open set $V_p(\alpha)$, then after applying an infinitesimally small translation and rotation, the intersection is still contained within $V_p(\alpha)$. Since $V_p(\alpha)$ is an open set, $\forall p \in \mathcal{P}_{AB}(\alpha \mid \psi)$ there exists an open neighborhood around $p$ that is a subset of $V_p(\alpha)$. Additionally, the compactness of $\mathcal{P}_{AB}(\alpha \mid \psi)$ implies that a finite subset of the union of those neighborhoods covers $\mathcal{P}_{AB}(\alpha \mid \psi)$. After applying an infinitesimally small transformation to $p$, it should stay in that finite cover because the change in distance between the origin and the point $p$ is Lipschitz continuous~\cite{GilbertJ85}. For LHC, we consider an arbitrary open set $\bar{V}$ such that $\Gamma(\psi) \cap \bar{V} \neq \emptyset$, i.e., with $p \in \mathcal{P}_{AB}(\alpha \mid \psi)$, $\bar{V}_p(\alpha)$ being an open set on $\mathbb{R}^3$, $\bar{V}_\alpha$ an open set on $\mathbb{R}$, and $\alpha \in S$, we have
\begin{equation}
    \bar{V} = \Big\{(p, \alpha) \mid \bar{V}_\alpha \cap S \neq \emptyset, \mathcal{P}_{AB}(\alpha \mid \psi) \cap \bar{V}_p(\alpha) \neq \emptyset\Big\}.
\end{equation}
In our case, LHC is equivalent to: for $\alpha \in \bar{V}_\alpha$, if $\mathcal{P}_{AB}(\alpha \mid \psi) \cap \bar{V}_p(\alpha) \neq \emptyset$, then after applying an infinitesimally small translation and rotation, the intersection set is not empty. Since there exists $p \in \mathcal{P}_{AB}(\alpha \mid \psi)$ with an open neighborhood that belongs to $\bar{V}_p(\alpha)$, following the logic for showing UHC, $\Gamma$ is also LHC. Thus, since $\Gamma(\psi)$ is a compact-valued correspondence, using Theorem~\ref{thm:berge}, we know $J^\star = \alpha^\star$ is a continuous function with respect to $\psi$.
\end{proof}

==> proof.tex <==
To show~\eqref{eq:diffopt_cbf} is a valid CBF, we show $\alpha^\star$ is a continuous function w.r.t. $(r_1, q_1, r_2, q_2)$ and provide conditions that~\eqref{eq:diffopt_cbf} is continuously differentiable as a conjecture. The discussion regarding $\partial h/\partial x \neq 0$ for $x\in\partial\mathcal{C}$ is provided in Section~\ref{sec:cbf_constraint}. First, we state one of the main theoretical results.
% Theorem 1
\begin{thm}
\label{thm:main}
The optimal value of~\eqref{eq:differentiable_collision}, denoted as $\alpha^\star$, is a continuous function with respect to the positions and orientations of $A$ and $B$.
\end{thm}
While the continuity of $\alpha^\star$ is proved later in this section, proving its continuous differentiability with respect to the link pose is more involved. Based on empirical studies, we believe that continuous differentiability holds under appropriate conditions motivating the conjecture below.
% Conjecture 1
\begin{conj}
\label{conj:cbf_condition}
Assume we have two convex objects $A$ and $B$. If $A$ is a strongly convex object (e.g., ellipsoid, sphere) and $B$ is a convex object that can either have a non-smooth surface (e.g., cylinder, polygon, cone) or a smooth surface, then the CBF defined in~\eqref{eq:diffopt_cbf} is continuously differentiable.
\end{conj}
Further analysis/proof of Conjecture~\ref{conj:cbf_condition} is deferred to future works. However, in Section~\ref{sec:robot_arm_exp}, we empirically show that even when continuous differentiability is not satisfied globally, the approach can still be implemented in practice on robotic systems and safety can be achieved. In the remainder of this section, we present the proof for Theorem~\ref{thm:main}. The main theoretical tool utilized in the proof of Theorem~\ref{thm:main} is Berge's Maximum Theorem:

\begin{thm}[Berge's Maximum Theorem~\cite{Border85}]
\label{thm:berge}
Let $X$ and $\Psi$ be topological spaces, and $J:X\times\Psi \rightarrow \mathbb{R}$ be a continuous function on $X\times\Psi$ and $\Gamma: \Psi\rightrightarrows X$ be a compact-valued correspondence such that $\Gamma(\psi) \neq \emptyset$ for all $\psi\in\Psi$. Define the value function $\mathcal{J}^\star: \Psi \rightarrow \mathbb{R}$ as
\begin{equation}
    \mathcal{J}^\star(\psi) = \sup\{\mathcal{J}(x, \psi) \mid x \in \Gamma(\psi)\}
\end{equation}
and the solution function $\Gamma^\star: \Psi \rightarrow X$ as
\begin{equation}
    \Gamma^\star(\psi) = \{x \mid x \in \Gamma(\psi), \mathcal{J}(x, \psi) = \mathcal{J}^\star(\psi)\}.
\end{equation}
If $\Gamma$ is an upper hemicontinuous (UHC) and lower hemicontinuous (LHC) correspondence at $\psi$, then $\mathcal{J}^\star$ is continuous, and $\Gamma^\star$ is UHC with nonempty and compact values.
\end{thm}

\noindent Correspondences, UHC, and LHC are defined as:
\begin{defn}[Correspondence, UHC, and LHC~\cite{Border85}]
A \textit{\textbf{correspondence}} (set-valued function) $\Gamma: \Psi \rightrightarrows X$ is said to be \textit{\textbf{UHC}} at $\psi$ if, for any open set $V \subseteq X$ with $\Gamma(\psi) \subset V$, there exists an open set $U$ such that for all $\bar{\psi} \in U$, $\Gamma(\bar{\psi}) \subset V$. A correspondence $\Gamma: \Psi \rightrightarrows X$ is said to be \textit{\textbf{LHC}} at $\psi$ if, for any open set $V \subseteq X$ with $\Gamma(\psi) \cap V \neq \emptyset$, there exists an open set $U$ such that for all $\bar{\psi} \in U$, $\Gamma(\bar{\psi}) \cap V \neq \emptyset$.
\end{defn}

For~\eqref{eq:differentiable_collision}, we have $(p, \alpha) \in X \subset \mathbb{R}^4$ and $\psi = (r_1, q_1, r_2, q_2) \in \Psi \subset \mathrm{SE}(3)\times\mathrm{SE}(3)$. The constraint correspondence $\Gamma(\psi)$ is defined as
\begin{equation}
    \Gamma(\psi) = \{(p, \alpha)\mid p \in \mathcal{P}_{AB}(\alpha \mid \psi), \alpha \in S\}
    \label{eq:constraint_correspondence}
\end{equation}
with $S \subset \mathbb{R}$ being a compact set and $\mathcal{P}_{AB}(\alpha \mid \psi) = \mathcal{P}_{A}(\alpha \mid \psi) \cap \mathcal{P}_B(\alpha \mid \psi)$. Also we define $\Gamma_i(\psi) = \{(p,\alpha) \mid p\in\mathcal{P}_i(\alpha\mid\psi), \alpha \in S\}$ with $i \in \{A, B\}$. We can then show that $\Gamma(\psi)$ is a compact-valued correspondence on $\mathbb{R}^4$.
\begin{lem}
The constraint correspondence $\Gamma(\psi)$ defined in~\eqref{eq:constraint_correspondence} is a compact-valued correspondence.
\end{lem}
\begin{proof}
First, we show that $\Gamma_A(\psi)$ is a compact-valued correspondence. Define $K_A(\psi) = \mathcal{P}_A(1\mid\psi) \subset \mathbb{R}^3$, and the function $\phi: K_A(\psi) \times S \rightarrow \mathbb{R}^4$ as $\phi(p, \alpha) = (\alpha(p - r_1) + r_1, \alpha)$, which is a continuous function on $K_A(\psi) \times S$. Because both $K_A(\psi)$ and $S$ are compact sets, we have $K_A(\psi) \times S$ as a compact set on $\mathbb{R}^4$. Since the image of $\psi$ under $\Gamma_A$ is the same as the image of $K_A(\psi) \times S$ under $\phi$, using the property that continuous functions map compact sets to compact sets, and $K_A(\psi)$ is a compact set for any value of $\psi$, we have $\Gamma_A(\psi)$ being a compact-valued correspondence. Using the same logic, for all $\psi$, $\Gamma_B(\psi)$ is also a compact-valued correspondence. Since $\Gamma(\psi) = \Gamma_A(\psi) \cap \Gamma_B(\psi)$, and intersections of compact sets are compact sets, we can conclude that $\Gamma(\psi)$ is a compact-valued correspondence.
\end{proof}

With the previous derivations, to directly apply Berge's Maximum Theorem to our problem, the only remaining assumption that needs to be verified is whether $\Gamma(\psi)$ is both UHC and LHC. We show this using the following proof: 

\begin{proof}
To show UHC using Theorem~\ref{thm:berge}, we consider an arbitrary open set $V$ such that that $\Gamma(\psi) \subset V$, i.e.,
\begin{equation}
    V = \Big\{(p, \alpha) \mid \mathcal{P}_{AB}(\alpha \mid \psi) \subset V_p(\alpha), S \subset V_\alpha\Big\}
\end{equation}
with $V_p$ being an open set on $\mathbb{R}^3$, $p \in \mathcal{P}_{AB}(\alpha \mid \psi)$, $V_\alpha$ being an open set on $\mathbb{R}$, and $\alpha \in S$. In our case, UHC is equivalent to: for any $\psi$ and $\alpha$, if the intersection of the two convex shapes $\mathcal{P}_A$ and $\mathcal{P}_B$ are contained within an open set $V_p(\alpha)$, then after applying an infinitesimally small translation and rotation, the intersection is still contained within $V_p(\alpha)$. Since $V_p(\alpha)$ is an open set, $\forall p \in \mathcal{P}_{AB}(\alpha \mid \psi)$ there exists an open neighborhood around $p$ that is a subset of $V_p(\alpha)$. Additionally, the compactness of $\mathcal{P}_{AB}(\alpha \mid \psi)$ implies that a finite subset of the union of those neighborhoods covers $\mathcal{P}_{AB}(\alpha \mid \psi)$. After applying an infinitesimally small transformation to $p$, it should stay in that finite cover because the change in distance between the origin and the point $p$ is Lipschitz continuous~\cite{GilbertJ85}. For LHC, we consider an arbitrary open set $\bar{V}$ such that $\Gamma(\psi) \cap \bar{V} \neq \emptyset$, i.e., with $p \in \mathcal{P}_{AB}(\alpha \mid \psi)$, $\bar{V}_p(\alpha)$ being an open set on $\mathbb{R}^3$, $\bar{V}_\alpha$ an open set on $\mathbb{R}$ and $\alpha \in S$ we have
\begin{equation}
    \bar{V} = \Big\{(p, \alpha) \mid \bar{V}_\alpha \cap S \neq \emptyset, \mathcal{P}_{AB}(\alpha \mid \psi) \cap \bar{V}_p(\alpha) \neq \emptyset\Big\}.
\end{equation}
In our case, LHC is equivalent to: for $\alpha \in \bar{V}_\alpha$, if $\mathcal{P}_{AB}(\alpha \mid \psi)$ intersects with an open set $\bar{V}_p(\alpha)$, then after applying an infinitesimally small translation and rotation, the intersection set is not empty. Since there exists $p \in \mathcal{P}_{AB}(\alpha \mid \psi)$ with an open neighborhood that belongs to $\bar{V}_p(\alpha)$, following the logic for showing UHC, $\Gamma$ is also LHC. Thus, by direct application of Theorem~\ref{thm:berge}, we know $J^\star = \alpha^\star$ is a continuous function with respect to $\psi$.
\end{proof}
